Every Answer Matters: Evaluating Commonsense with Probabilistic Measures

Large language models have demonstrated impressive performance on commonsense tasks; however, these tasks are often posed as multiple-choice questions, allowing models to exploit systematic biases. Commonsense is also inherently probabilistic with multiple correct answers. The purpose of "boiling water" could be making tea and cooking, but it also could be killing germs. Existing tasks do not capture the probabilistic nature of common sense. To this end, we present commonsense frame completion (CFC), a new generative task that evaluates common sense via multiple open-ended generations. We also propose a method of probabilistic evaluation that strongly correlates with human judgments. Humans drastically outperform strong language model baselines on our dataset, indicating this approach is both a challenging and useful evaluation of machine common sense.

==> figures/protoqa_sample_figure.tex <==
\begin{figure*}[!tbp]
  \centering
  \begin{minipage}{0.45\textwidth}
    \includegraphics[width=\textwidth]{Image/scatter_plot_protoQA_centered_protoqa_dev.png}
  \end{minipage}
  \hfill
  \begin{minipage}{0.45\textwidth}
    \includegraphics[width=\textwidth]{Image/scatter_plot_centered_protoqa_dev.png}
  \end{minipage}
  \caption{Comparison of correlation between ProtoQA evaluator and CFC evaluator for sampled questions in ProtoQA dev with ground-truth clusters. The X-axis is the evaluaotr score with human assignment, and the y-axis is the KL value with WordNet assignment. The figure on the left is the correlation for ProtoQA Max-10 with human clustering and WordNet matching. The figure on the right is the correlation for CFC evaluator with human clustering and WordNet matching. TThese corresponds to the ProtoQA evaluator / Human / WordNet column and the CFC evaluator / Human / WordNet rows with the column being CFC dev in Table \ref{tab:correlation-dev}. Different questions are annotated with different colors.}
\label{fig:scatter_protoQA}
\end{figure*}

